Fair Termination of Asynchronous Binary Sessions

We study a theory of asynchronous session types ensuring that well-typed processes terminate under a suitable fairness assumption. Fair termination entails starvation freedom and orphan message freedom namely that all messages, including those that are produced early taking advantage of asynchrony, are eventually consumed. The theory is based on a novel fair asynchronous subtyping relation for session types that is coarser than the existing ones. The type system is also the first of its kind that is firmly rooted in linear logic: fair asynchronous subtyping is incorporated as a natural generalization of the cut and axiom rules of linear logic and asynchronous communication is modeled through a suitable set of commuting conversions and of deep cut reductions in linear logic proofs.

==> other-subtypings.tex <==
\section{Other subtypings}

In this section we compare our subtyping with the other binary session subtypings in the literature.
To have a common syntax, we restrict to the first order fragment (e.g. the subtyping in 
\cite{BravettiLangeZavattaro24} is not higher-order) and we consider only
fairly terminating types (e.g. fair termination implies the notion
of controllable types used in the subtyping defined in \cite{BravettiLangeZavattaro24}).
\GZ{Sono già definiti o dobbiamo definire qui?} 
In the definition of our subtyping (see \cref{def:cas}), we have used the labeled transition system $\lred{}$
defined in \cref{tab:lts}, which includes early outputs and late inputs. 
Other subtypings consider less permissive transition systems. For this reason we consider 
the transitions $\lmust{}$ of immediate actions (obtained by considering only the 
\rulename{MUST-*} rules) and the transitions $\lind{}$ of bounded anticipated actions 
(obtained by considering only the one-line rules interpreted inductively). 

\begin{definition}[Gay-Hole \cite{GayHole05}]
  \label{def:GH}
  We say that $\srel$ is a \emph{synchronous subtyping} if $(S,T)
  \in \srel$ implies:
  \begin{enumerate}
  \item\label{cas:endGH} either $\positive(S)$ or $\negative(T)$;
  \item\label{cas:inpGH} if $T \lmust{\inp\MessageType} T'$ 
      then $S \lmust{\inp\MessageType} S'$
      and $(S',T') \in \srel$;
  \item\label{cas:outGH} if $S \lmust{\out\MessageType} S'$
      then $T \lmust{\out\MessageType} T'$
      and $(S',T') \in \srel$.
  \end{enumerate}
  We write $\ghsubt$ for the largest synchronous subtyping $\srel$.
\end{definition}

\begin{definition}[Mostrous-Yoshida \cite{MostrousYoshida15}]
  \label{def:MY}
  We say that $\srel$ is an \emph{asynchronous subtyping} if $(S,T)
  \in \srel$ implies:
  \begin{enumerate}
  \item\label{cas:endMY} either $\positive(S)$ or $\negative(T)$;
  \item\label{cas:inpMY} if $\negative(S)$ and $T \lmust{\inp\MessageType} T'$ 
      then $S \lmust{\inp\MessageType} S'$
      and $(S',T') \in \srel$;
  \item\label{cas:outMY} if $S \lmust{\out\MessageType} S'$ then $T
      \lind{\out\MessageType} T'$ and $(S',T') \in \srel$.
      
  \end{enumerate}
   We write $\mysubt$ for the largest asynchronous subtyping.
\end{definition}

\begin{definition}[Chen et al. \cite{ChenDezaniScalasYoshida17}]
  \label{def:M}
  We say that $\srel$ is an \emph{asynchronous orphan message free subtyping} if $(S,T)
  \in \srel$ implies:
  \begin{enumerate}
  \item\label{cas:endC} either $\positive(S)$ or $\negative(T)$;
  \item\label{cas:inpC} if $\negative(S)$ and $T \lmust{\inp\MessageType} T'$ then $S \lmust{\inp\MessageType} S'$
      and $(S',T') \in \srel$;
  \item if $S \lmust{\out\MessageType} S'$ then $T
      \lind{\out\MessageType} T'$ and $(S',T') \in \srel$ and either $T
      \lmust{\out\MessageType}$ or $S \lind{\inp\MessageTypeT}$.
  \end{enumerate}
  We write $\csubt$ for the largest asynchronous orphan message free 
  subtyping.
\end{definition}

*** LA PARTE QUI SOTTO SU BRAVETTI NON VA BENE, E' ANCORA TUTTA DA RIVEDERE **
The fair asynchronous subtyping proposed by Bravetti et al. \cite{BravettiLangeZavattaro24}
differs from the asynchronous subtyping of \cite{MostrousYoshida15} for two main reasons:
it allows for unbounded anticipation of outputs and it does not admit covariance of outputs.
Hence, in the rule about output actions, we use the transition $T \lred{\out\MessageType} T'$ instead
of $T \lind{\out\MessageType} T'$ and we also impose 
$\outputs(S)=\outputs(T)$, where $\outputs(R) = \{\MessageType \mid R \lred{\out\MessageType}\}$.


%allows for unbounded output anticipation, but only under the assumption that all initial
%subterms performing output actions have precisely the same output tags. Formally,
%we can obtain the same definition by considering a variant of our LTS of types in \cref{tab:lts}
%where we add the additional premise $\forall i,j \in I: \outputs(S_i)=\outputs(S_j)$ to the
%rule \rulename{MUST-$\oplus$}, where $\outputs(T) = \{\MessageType \mid T \lred{\out\MessageType}\}$.


\begin{definition}[Bravetti et al. \cite{BravettiLangeZavattaro24}]
  \label{def:B}
  We say that $\srel$ is a \emph{fair asynchronous subtyping} if $(S,T)
  \in \srel$ implies:
  \begin{enumerate}
  \item\label{cas:endB} either $\positive(S)$ or $\negative(T)$;
  \item\label{cas:inpB} if $T \lmust{\inp\MessageType} T'$ then $S \lmust{\inp\MessageType} S'$
      and $(S',T') \in \srel$;
  \item\label{cas:outB} if $S \lmust{\out\MessageType} S'$ then 
  $T \lred{\out\MessageType} T'$ and $(S',T') \in \srel$ and $\outputs(S)=\outputs(T)$.
%  $\{\MessageTypeT \mid S \lred{\out\MessageTypeT}\} = \{\MessageTypeT \mid T \lred{\out\MessageTypeT}\}$.
  \end{enumerate}
  We write $\bsubt$ for the largest fair asynchronous subtyping.
\end{definition}

***** DA QUI IN POI VA BENE *****

\begin{lemma}
  \label{lem:ftind}
  If $S$ is fairly terminating and $S \cored\Action T$, then $S \ired\Action T$.
  \GZ{La relazione con pedice coind non è definita}
\end{lemma}
\begin{proof}
  By induction on the minimum depth of a leaf in $S$, knowing that such depth is
  finite from the assumption that $S$ is fairly terminating, and by cases on the
  shape of $S$.
\end{proof}

\begin{lemma}
  \label{lem:my-inp}
  If $S \mysubt T$ and $T \lred{\inp\MessageType}$, then $S
  \lred{\inp\MessageType}$.
  ***** OPPPSSSS.. ANCHE QUESTO LEMMA E' FALSO PER $\One \mysubt \With{\Tag : \One}$.
  L'ERRORE NELLA PROOF E' NEL CASO $T = \With{\Tag_i : T_i}_{i\in I}$ QUANDO
  DICIAMO CHE $\positive(S)$ IMPLICA $S = \Plus{\Tag_j : S_j}_{j\in J}$. IN QUESTO
  CASO $S$ POTREBBE ANCHE ESSERE $\One$ *****
\end{lemma}
\begin{proof}
  Note that in this proof we treat $\lred{\inp\MessageType}$ as a unary
  predicate.
  %
  By \cref{lem:ftind} it is enough to show that $S \lred{\inp\MessageType}$ is
  \emph{coinductively} derivable using the singly-lines rules in \cref{tab:lts}.
  To this aim it suffices to show that
  \[
    \rrel \eqdef \set{ S \mid S \mysubt T \wedge T \lred{\inp\MessageType}}
  \]
  is backward closed with respect to the singly-lined rules in \cref{tab:lts}.
  %
  Let $S \in \rrel$. Then $S \mysubt T$ and $T \lred{\inp\MessageType}$ for some
  $T$. We reason by cases on the shape of $T$ to show that $S
  \lred{\inp\MessageType}$ is the conclusion of one of the rules in
  \cref{tab:lts}.

  \proofcase{$T = \Bot$}
  %
  Then $\MessageType = \unit$ and $T \lmust{\inp\unit}$.
  %
  $\positive(S)$ does not hold, otherwise $S \lmust{\out\MessageTypeT} S'$ which
  implies, by \cref{def:MY}\eqref{cas:outMY},  $T \lind{\out\MessageTypeT} T'$
  that does not hold because $T = \Bot$. 
  %
  Hence $\negative(S)$. We deduce, by \cref{def:MY}\eqref{cas:inpMY},
  that $S \xlmust{\inp\unit}$, hence $S \xlred{\inp\unit}$.

  \proofcase{$T = \With{\Tag_i : T_i}_{i\in I}$}
  %
  Then $\MessageType = \Tag_k$ for some $k\in I$ and $T \lmust{\inp\Tag_k}$.
  %
  There are two possible cases: either $\negative(S)$ or $\positive(S)$. 
  %
  If $\negative(S)$, from \cref{def:MY}\eqref{cas:inpMY} we deduce $S \xlmust{\inp\Tag_k}$, hence $S
  \xlred{\inp\Tag_k}$.
  %
  If $\positive(S)$, then $S = \Plus{\Tag_j : S_j}_{j\in J}$.
  From \cref{def:MY}\eqref{cas:outMY} we deduce that, for each $j \in J$,
  there exists $T \lind{\out\Tag_j} T_j$ s.t. $S_j \mysubt T_j$.
  We have that $T_j = \With{\Tag_i : T'_i}_{i\in I}$; from
  $\MessageType = \Tag_k$ for some $k\in I$ we conclude $T_j \lmust{\inp\MessageType}$
  hence also $T_j \lred{\inp\MessageType}$.
  By $S_j \mysubt T_j$ and $T_j \lred{\inp\MessageType}$ we have $S_j \in \rrel$ for every 
  $j \in J$ by definition of $\rrel$. We conclude by observing that $S \lred{\inp\MessageType}$ 
  is the conclusion of \APlusT.  
  
  \proofcase{$T = \Plus{\Tag_i : T_i}_{i\in I}$}
  %
  Then $T_i \lred{\inp\MessageType}$ for every $i\in I$.
  %
  From $S \mysubt T$ we deduce $\positive(S)$, hence $S = \Plus{\Tag_i :
  S_i}_{i\in J}$ and $J \subseteq I$ and $S_i \mysubt T_i$ for every $i\in J$.
  %
  Now we have $S_i \in \rrel$ for every $i\in J$ by definition of $\rrel$ and we
  conclude by observing that $S \lred{\inp\MessageType}$ is the conclusion of
  \APlusT.
\end{proof}


\begin{lemma}
  \label{lem:my-inp-subt}
  If $S \mysubt T$ and $T \lred{\inp\MessageType} T'$, then $S
  \lred{\inp\MessageType} S'$ and $S' \mysubt T'$.
\end{lemma}
\begin{proof}
  It suffices to show that
  \[
    \srel \eqdef {\mysubt} \cup \set{ (S', T') \mid S \mysubt T \wedge S \lred{\inp\MessageType} S' \wedge T \lred{\inp\MessageType} T'}
  \]
  satisfies the clauses of \cref{def:MY}. Clearly any pair of types in $\mysubt$
  satisfies those clauses, so consider $(S',T') \in \srel$ such that $S \mysubt
  T$ and $S \lred{\inp\MessageType} S'$ and $T \lred{\inp\MessageType} T'$.
  %
  We reason by cases on the shape of $T$.

  \proofcase{$T = \Bot$}
  %
  Then $\MessageType = \unit$ and $T' = \Bot$ and $T \lmust{\inp\unit} T'$.
  %
  $\positive(S)$ does not hold, otherwise $S \lmust{\out\MessageTypeT} S'$ which
  implies, by \cref{def:MY}\eqref{cas:outMY},  $T \lind{\out\MessageTypeT} T'$
  that does not hold because $T = \Bot$.
  From \cref{def:MY}\eqref{cas:inpMY} we deduce $S \lmust{\inp\unit} S'$ and $S'
  \mysubt T'$ and we conclude by observing that $(S',T') \in \srel$.

  \proofcase{$T = \With{\Tag_i : T_i}_{i\in I}$}
  %
  Then $\MessageType = \Tag_k$ and $T' = T_k$ and $T \lmust{\inp\Tag_k} T'$ for
  some $k\in I$.
  %
  There are two possible cases: either $\negative(S)$ or $\positive(S)$. 
  %
  If $\negative(S)$, from $S \mysubt T$ we deduce $S = \With{\Tag_i : S_i}_{i\in J}$ and $I
  \subseteq J$ and $S_i \mysubt T_i$ for every $i \in I$.
  %
  Also, $S' = S_k$.
  %
  We observe that $S \lmust{\inp\Tag_k} S'$ and that $(S',T') \in
  \srel$ by definition of $\srel$.
  %
  If $\positive(S)$, then $S = \Plus{\Tag_j : S_j}_{j\in J}$.
  We observe $S' = \Plus{\Tag_j : S_j'}_{j\in J}$ with $S_j'$ s.t.
  $S_j \lred{\inp\MessageType} S_j'$. We need to show that, for every $j\in J$,
  $T_k \lind{\out\Tag_j} T_{kj}$ and $(S_j',T_{kj}) \in \srel$.
  %
  From $S \mysubt T$, we have that $T \lind{\out\Tag_j} T_j$ for every $j\in J$
  and $S_j \mysubt T_j$ with $T_j = \With{\Tag_i : T_{ij}}_{i\in I}$ with 
  $T_i \lind{\out\Tag_j} T_{ij}$ (hence also $T_i \lred{\out\Tag_j} T_{ij}$).
  Hence for every $j \in J$ we have $S_j \mysubt T_j$, $S_j \lred{\inp\MessageType} S_j'$ and 
  $T_j \lred{\inp\MessageType} T_{kj}$ (because $\MessageType = \Tag_k$)
  from which we conclude that $(S_j',T_{kj}) \in \srel$ by definition of $\srel$.

  \proofcase{$T = \Plus{\Tag_i : T_i}_{i\in I}$}
  %
  Then $T_i \lred{\inp\MessageType} T_i'$ for every $i\in I$ and $T' =
  \Plus{\Tag_i : T_i'}_{i\in I}$.
  %
  From $S \mysubt T$ we deduce $\positive(S)$. Hence $S = \Plus{\Tag_i : S_i}_{i\in J}$ and $J
  \subseteq I$ and $S_i \mysubt T_i$ for every $i\in J$.
  %
  From \cref{lem:my-inp} we deduce $S_i \lred{\inp\MessageType} S_i'$ for every
  $i\in J$.
  %
  We conclude by observing that $(S_i', T_i') \in \srel$ by definition of
  $\srel$.
\end{proof}



\begin{lemma}
  \label{lem:my-out}
  If $S \mysubt T$ and $S \lred{\out\MessageType}$, then 
  $T \lred{\out\MessageType}$.
\end{lemma}
\begin{proof}
  Note that in this proof we treat $\lred{\out\MessageType}$ as a unary
  predicate.
  %
  By \cref{lem:ftind} it is enough to show that $S \lred{\out\MessageType}$ is
  \emph{coinductively} derivable using the singly-lines rules in \cref{tab:lts}.
  To this aim it suffices to show that
  \[
    \rrel \eqdef \set{ T \mid S \mysubt T \wedge S \lred{\out\MessageType}}
  \]
  is backward closed with respect to the singly-lined rules in \cref{tab:lts}.
  %
  Let $T \in \rrel$. Then $S \mysubt T$ and $S \lred{\out\MessageType}$ for some
  $S$. We reason by cases on the shape of $S$ to show that $T
  \lred{\out\MessageType}$ is the conclusion of one of the rules in
  \cref{tab:lts}.

  \proofcase{$S = \One$}
  %
  Then $\MessageType = \unit$ and $S \lmust{\out\unit}$.
  %
  $\negative(T)$ does not hold, otherwise $T \lmust{\inp\MessageTypeT} T'$ which
  implies, by \cref{def:MY}\eqref{cas:inpMY},  $S \lmust{\inp\MessageTypeT} S'$
  that does not hold because $S = \One$. 
  ****** OPPPPSSSS... POTREMMO AVERE $\One \mysubt \With{\Tag : \One}$ 
  TUTTO DA RICONTROLLARE!!!!! ******
  %
  Hence $\positive(T)$. We deduce, by \cref{def:MY}\eqref{cas:outMY},
  that $T \lind{\out\unit}$, hence $T \xlred{\out\unit}$.

  \proofcase{$S = \With{\Tag_i : S_i}_{i\in I}$}
  %
  Then $S_i \lred{\out\MessageType}$ for every $i\in I$.
  %
  From $S \mysubt T$ we deduce $\negative(T)$, hence $T = \With{\Tag_i :
  T_i}_{i\in J}$ and $J \subseteq I$ and $S_i \mysubt T_i$ for every $i\in J$.
  %
  Now we have $T_i \in \rrel$ for every $i\in J$ by definition of $\rrel$ and we
  conclude by observing that $T \lred{\out\MessageType}$ is the conclusion of
  \AWithT.
  
  \proofcase{$S = \Plus{\Tag_i : S_i}_{i\in I}$}
  %
  Then $\MessageType = \Tag_k$ for some $k\in I$ and $S \lmust{\out\Tag_k}$.
  %
  From \cref{def:MY}\eqref{cas:outMY} we deduce $T \lind{\out\Tag_k}$, hence also 
  $T \lred{\out\MessageType}$ because $\MessageType = \Tag_k$.
\end{proof}


\begin{lemma}
  \label{lem:my-out-subt}
  If $S \mysubt T$ and $S \lred{\out\MessageType} S'$, then $T
  \lred{\out\MessageType} T'$ and $S' \mysubt T'$.
\end{lemma}
\begin{proof}
  It suffices to show that
  \[
    \srel \eqdef {\mysubt} \cup \set{ (S', T') \mid S \mysubt T \wedge S \lred{\out\MessageType} S' \wedge T \lred{\out\MessageType} T'}
  \]
  satisfies the clauses of \cref{def:MY}. Clearly any pair of types in $\mysubt$
  satisfies those clauses, so consider $(S',T') \in \srel$ such that $S \mysubt
  T$ and $S \lred{\out\MessageType} S'$ and $T \lred{\out\MessageType} T'$.
  %
  We reason by cases on the shape of $T$.

  \proofcase{$T = \One$}
  %
  Then $\MessageType = \unit$ and $T' = \One$ and $S \lmust{\out\unit} S'$.
  %
  $\negative(T)$ does not hold, otherwise $T \lmust{\inp\MessageTypeT} T'$ which
  implies, by \cref{def:MY}\eqref{cas:inpMY},  $T \lind{\out\MessageTypeT} T'$
  that does not hold because $T = \Bot$.
  From \cref{def:MY}\eqref{cas:inpMY} we deduce $S \lmust{\inp\unit} S'$ and $S'
  \mysubt T'$ and we conclude by observing that $(S',T') \in \srel$.

  \proofcase{$T = \With{\Tag_i : T_i}_{i\in I}$}
  %
  Then $\MessageType = \Tag_k$ and $T' = T_k$ and $T \lmust{\inp\Tag_k} T'$ for
  some $k\in I$.
  %
  There are two possible cases: either $\negative(S)$ or $\positive(S)$. 
  %
  If $\negative(S)$, from $S \mysubt T$ we deduce $S = \With{\Tag_i : S_i}_{i\in J}$ and $I
  \subseteq J$ and $S_i \mysubt T_i$ for every $i \in I$.
  %
  Also, $S' = S_k$.
  %
  We observe that $S \lmust{\inp\Tag_k} S'$ and that $(S',T') \in
  \srel$ by definition of $\srel$.
  %
  If $\positive(S)$, then $S = \Plus{\Tag_j : S_j}_{j\in J}$.
  We observe $S' = \Plus{\Tag_j : S_j'}_{j\in J}$ with $S_j'$ s.t.
  $S_j \lred{\inp\MessageType} S_j'$. We need to show that, for every $j\in J$,
  $T_k \lind{\out\Tag_j} T_{kj}$ and $(S_j',T_{kj}) \in \srel$.
  %
  From $S \mysubt T$, we have that $T \lind{\out\Tag_j} T_j$ for every $j\in J$
  and $S_j \mysubt T_j$ with $T_j = \With{\Tag_i : T_{ij}}_{i\in I}$ with 
  $T_i \lind{\out\Tag_j} T_{ij}$ (hence also $T_i \lred{\out\Tag_j} T_{ij}$).
  Hence for every $j \in J$ we have $S_j \mysubt T_j$, $S_j \lred{\inp\MessageType} S_j'$ and 
  $T_j \lred{\inp\MessageType} T_{kj}$ (because $\MessageType = \Tag_k$)
  from which we conclude that $(S_j',T_{kj}) \in \srel$ by definition of $\srel$.

  \proofcase{$T = \Plus{\Tag_i : T_i}_{i\in I}$}
  %
  Then $T_i \lred{\inp\MessageType} T_i'$ for every $i\in I$ and $T' =
  \Plus{\Tag_i : T_i'}_{i\in I}$.
  %
  From $S \mysubt T$ we deduce $\positive(S)$. Hence $S = \Plus{\Tag_i : S_i}_{i\in J}$ and $J
  \subseteq I$ and $S_i \mysubt T_i$ for every $i\in J$.
  %
  From \cref{lem:my-inp} we deduce $S_i \lred{\inp\MessageType} S_i'$ for every
  $i\in J$.
  %
  We conclude by observing that $(S_i', T_i') \in \srel$ by definition of
  $\srel$.
\end{proof}




\subsection{General Results}

%\begin{lemma}
%  \label{lem:ftind}
%  If $S$ is fairly terminating and $S \cored\Action T$, then $S \ired\Action T$.
%  \GZ{La relazione con pedice coind non è definita}
%\end{lemma}
%\begin{proof}
%  By induction on the minimum depth of a leaf in $S$, knowing that such depth is
%  finite from the assumption that $S$ is fairly terminating, and by cases on the
%  shape of $S$.
%\end{proof}

\subsection{${\ghsubt} \subseteq {\subt}$}

%\begin{lemma}
%  \label{lem:gh-inp}
%  If $S \ghsubt T$ and $T \lred{\inp\MessageType}$, then $S
%  \lred{\inp\MessageType}$.
%\end{lemma}
%\begin{proof}
%  Note that in this proof we treat $\lred{\inp\MessageType}$ as a unary
%  predicate.
%  %
%  By \cref{lem:ftind} it is enough to show that $S \lred{\inp\MessageType}$ is
%  \emph{coinductively} derivable using the singly-lines rules in \cref{tab:lts}.
%  To this aim it suffices to show that
%  \[
%    \rrel \eqdef \set{ S \mid S \ghsubt T \wedge T \lred{\inp\MessageType}}
%  \]
%  is backward closed with respect to the singly-lined rules in \cref{tab:lts}.
%  %
%  Let $S \in \rrel$. Then $S \ghsubt T$ and $T \lred{\inp\MessageType}$ for some
%  $T$. We reason by cases on the shape of $T$ to show that $S
%  \lred{\inp\MessageType}$ is the conclusion of one of the rules in
%  \cref{tab:lts}.
%
%  \proofcase{$T = \Bot$}
%  %
%  Then $\MessageType = \unit$ and $T \lmust{\inp\unit}$.
%  %
%  From \cref{def:GH} we deduce $S \xlmust{\inp\unit}$, hence $S
%  \xlred{\inp\unit}$.
%
%  \proofcase{$T = \With{\Tag_i : T_i}_{i\in I}$}
%  %
%  Then $\MessageType = \Tag_k$ for some $k\in I$ and $T \lmust{\inp\Tag_k}$.
%  %
%  From \cref{def:GH} we deduce $S \xlmust{\inp\Tag_k}$, hence $S
%  \xlred{\inp\Tag_k}$.
%
%  \proofcase{$T = \Plus{\Tag_i : T_i}_{i\in I}$}
%  %
%  Then $T_i \lred{\inp\MessageType}$ for every $i\in I$.
%  %
%  From $S \ghsubt T$ we deduce $\positive(S)$, hence $S = \Plus{\Tag_i :
%  S_i}_{i\in J}$ and $J \subseteq I$ and $S_i \ghsubt T_i$ for every $i\in J$.
%  %
%  Now we have $S_i \in \rrel$ for every $i\in J$ by definition of $\rrel$ and we
%  conclude by observing that $S \lred{\inp\MessageType}$ is the conclusion of
%  \APlusT.
%\end{proof}

\begin{lemma}
  \label{lem:gh-inp-subt}
  If $S \ghsubt T$ and $T \lred{\inp\MessageType} T'$, then $S
  \lred{\inp\MessageType} S'$ and $S' \ghsubt T'$.
\end{lemma}
\begin{proof}
  It suffices to show that
  \[
    \srel \eqdef {\ghsubt} \cup \set{ (S', T') \mid S \ghsubt T \wedge S \lred{\inp\MessageType} S' \wedge T \lred{\inp\MessageType} T'}
  \]
  satisfies the clauses of \cref{def:GH}. Clearly any pair of types in $\ghsubt$
  satisfies those clauses, so consider $(S',T') \in \srel$ such that $S \ghsubt
  T$ and $S \lred{\inp\MessageType} S'$ and $T \lred{\inp\MessageType} T'$.
  %
  We reason by cases on the shape of $T$.

  \proofcase{$T = \Bot$}
  %
  Then $\MessageType = \unit$ and $T' = \Bot$ and $T \lmust{\inp\unit} T'$.
  %
  From \cref{def:GH}\eqref{cas:inpGH} we deduce $S \lmust{\inp\unit} S'$ and $S'
  \ghsubt T'$ and we conclude by observing that $(S',T') \in \srel$.

  \proofcase{$T = \With{\Tag_i : T_i}_{i\in I}$}
  %
  Then $\MessageType = \Tag_k$ and $T' = T_k$ and $T \lmust{\inp\Tag_k} T'$ for
  some $k\in I$.
  %
  From $S \ghsubt T$ we deduce $S = \With{\Tag_i : S_i}_{i\in J}$ and $I
  \subseteq J$ and $S_i \ghsubt T_i$ for every $i \in I$.
  %
  Also, $S' = S_k$.
  %
  We conclude by observing that $S \lmust{\inp\Tag_k} S'$ and that $(S',T') \in
  \srel$ by definition of $\srel$.

  \proofcase{$T = \Plus{\Tag_i : S_i}_{i\in I}$}
  %
  Then $T_i \lred{\inp\MessageType} T_i'$ for every $i\in I$ and $T' =
  \Plus{\Tag_i : T_i'}_{i\in I}$.
  %
  From $S \ghsubt T$ we deduce $S = \Plus{\Tag_i : S_i}_{i\in J}$ and $J
  \subseteq I$ and $S_i \ghsubt T_i$ for every $i\in J$.
  %
  From \cref{lem:gh-inp} we deduce $S_i \lred{\inp\MessageType} S_i'$ for every
  $i\in J$.
  %
  We conclude by observing that $(S_i', T_i') \in \srel$ by definition of
  $\srel$.
\end{proof}

\begin{lemma}
  \label{lem:gh-out-subt}
  If $S \ghsubt T$ and $S \lred{\out\MessageType} S'$, then $T
  \lred{\out\MessageType} T'$ and $S' \ghsubt T'$.
\end{lemma}
\begin{proof}
  Since $\ghsubt$ is closed under duality, from $S \ghsubt T$ we deduce
  $\dual{T} \ghsubt \dual{S}$.
  %
  Since the LTS is symmetric and we are considering first-order session types
  only, from $S \lred{\out\MessageType} S'$ we deduce $\dual{S}
  \lred{\inp\MessageType} \dual{S'}$.
  %
  Using \cref{lem:gh-inp-subt} we deduce $\dual{T} \lred{\inp\MessageType}
  \dual{T'}$ and $\dual{T'} \ghsubt \dual{S'}$, that is $S' \ghsubt T'$.
\end{proof}

\begin{theorem}
  \label{thm:ghsubt}
  If $S \ghsubt T$, then $S \subt T$.
\end{theorem}
\begin{proof}
  It suffices to show that $(S,T)$ satisfies the clauses of \cref{def:cas}.
  %
  From $S \ghsubt T$ and \cref{def:GH}\eqref{cas:endGH} we deduce either
  $\positive(S)$ or $\negative(T)$, hence~\rcas{pol} is satisfied.
  %
  Suppose $T \lred{\inp\MessageType} T'$.
  %
  From \cref{lem:gh-inp-subt} we deduce $S \lred{\inp\MessageType} S'$ and $S'
  \ghsubt T'$, hence~\rcas{inp} is satisfied.
  %
  Suppose $S \lred{\out\MessageType} S'$.
  %
  From \cref{lem:gh-out-subt} we deduce $T \lred{\out\MessageType} T'$ and $S'
  \ghsubt T'$, hence~\rcas{out} is satisfied.
\end{proof}

==> subtyping-mostrous-yoshida.tex <==

\clearpage
\color{purple}
\section{Subtyping di Mostrous-Yoshida}

\newcommand\emy{\subt^{\mathsf{eleg}}_{\mathsf{MY}}}
\newcommand\umy{\subt^{\mathsf{ugly}}_{\mathsf{MY}}}

\begin{definition}[Mostrous-Yoshida \cite{MostrousYoshida15}]
    \label{def:umy}
    We say that $\srel$ is an \emph{ugly asynchronous subtyping} if $(S,T) \in
    \srel$ implies:
    \begin{enumerate}
    \item\label{umy:pol} if $S \lmust{\pol\unit}$ then $T \lmust{\pol\unit}$;
    \item\label{umy:inp} if $S \lmust{\inp\TagB}$ then $T \lmust{\inp\TagC}$ and
        ($T \lmust{\inp\Tag} T'$ implies $S \lmust{\inp\Tag} S'$ and $(S',T')
        \in \srel$);
    \item\label{umy:out} if $S \lmust{\out\Tag} S'$ then $T \lind{\out\Tag} T'$
        and $(S',T') \in \srel$.
    \end{enumerate}
        We write $\umy$ for the largest ugly asynchronous subtyping.
\end{definition}

\newcommand\umyref[1]{Clause~\ref{def:umy}(\ref{umy:#1})}
\newcommand\emyref[1]{Clause~\ref{def:emy}(\ref{emy:#1})}

\begin{theorem}
    ${\emy} \subseteq {\umy}$
\end{theorem}
\begin{proof}
    We show that $\emy$ is an ugly coinductive subtyping assuming $S \emy T$ and
    proving the clauses of \cref{def:umy} in order:
    \begin{enumerate}
    \item Suppose $S \lmust{\pol\unit}$. We distinguish two sub-cases:
        \begin{itemize}
        \item ($\pol = \inp$) Then $\negative(S)$, hence $\negative(T)$. Suppose
            by contradiction that $T \lmust{\inp\Tag}$ for some $\Tag$. From
            \emyref{inp} we deduce $S \lind{\inp\Tag}$ which is incompatible
            with $S \lmust{\inp\unit}$. Therefore $T \lmust{\inp\unit}$ as
            required by \umyref{pol}.
        \item ($\pol = \out$) From \emyref{out} we deduce $T \lind{\out\unit}$.
            Suppose by contradiction that $T \lmust{\inp\Tag}$ for some $\Tag$.
            From \emyref{inp} we deduce $S \lind{\inp\Tag}$ which is
            incompatible with $S \lmust{\out\unit}$. Therefore $T
            \lmust{\out\unit}$ as required by \umyref{pol}.
        \end{itemize}
    \item Suppose $S \lmust{\inp\TagB}$. Then $\negative(S)$. From \emyref{pol}
        we deduce $\negative(T)$.
        %
        Suppose by contradiction $T \lmust{\inp\unit}$. Then from \emyref{inp}
        we deduce $S \lind{\inp\unit}$ which is incompatible with $S
        \lmust{\inp\TagB}$. Hence $T \lmust{\inp\TagC}$ for some $\TagC$ as
        required by \umyref{inp}.\LP{Forse qui stiamo assumendo che non ci siano
        i casi degeneri di scelte vuote.}
        %
        Now suppose $T \lmust{\inp\Tag} T'$. From \emyref{inp} we deduce $S
        \lind{\inp\Tag} S'$ and $S' \emy T'$. But then $S \lmust{\inp\Tag} S'$,
        as required by \umyref{inp}.
    \item Suppose $S \lmust{\out\Tag} S'$. From \emyref{out} we deduce $T
        \lind{\out\Tag} T'$ and $S' \emy T'$, therefore $S' \umy T'$ as required
        by \umyref{out}.
        %
        \qedhere
    \end{enumerate}
\end{proof}

\begin{lemma}
    \label{lem:umy-emy-late-input}
    If\/ $S \umy T$ and $T \lmust{\inp\Tag}$ then $S \lind{\inp\Tag}$.
\end{lemma}
\begin{proof}
    By induction on the minimum depth of a leaf in $S$. We know that this
    quantity is finite because of the assumption that $S$ is a fairly
    terminating session type.
    %
    If $\negative(S)$, suppose by contradiction $S \lmust{\inp\unit}$. From
    \umyref{pol} we deduce $T \lmust{\inp\unit}$, which contradicts the
    hypothesis $T \lmust{\inp\Tag}$. Hence $S \lmust{\inp\TagB}$ for some
    $\TagB$.\LP{E i casi degeneri con $\Zero$ e $\Top$? Forse sono da escludere.}
    %
    From \umyref{inp} we deduce $S \lmust{\inp\Tag}$, hence we conclude $S
    \lind{\inp\Tag}$.
    %
    If $\positive(S)$, suppose by contradiction $S \lmust{\out\unit}$. From
    \umyref{pol} we deduce $T \lmust{\out\unit}$, which contradicts the
    hypothesis $T \lmust{\inp\Tag}$. Hence $S \lmust{\out\TagB} S''$ for some
    $\TagB$.
    %
    Consider any $\TagC$ and $S''$ such that $S \lmust{\out\TagC} S''$. From
    \umyref{out} we deduce $T \lind{\out\TagC} T''$ and $S'' \umy T''$.
    %
    From $T \lmust{\inp\Tag} T'$ and $T \lind{\out\TagC} T''$ we deduce that
    $T'' \lmust{\inp\Tag} T'''$ for some $T'''$.
    %
    Now the minimum depth of a leaf in $S''$ is strictly smaller than the depth
    of a leaf in $S$, therefore we can use the induction hypothesis to deduce
    that $S'' \lind{\inp\Tag}$.
    %
    Since this is true for every $\TagC$ and $S''$ such that $S
    \lmust{\out\TagC} S''$ it must be the case that $S \lind{\inp\Tag}$.
\end{proof}

\begin{lemma}
    \label{lem:umy-emy-difficult-case}
    If $S \umy T$ and $S \lind{\inp\Tag} S'$ and $T \lmust{\inp\Tag} T'$, then
    $S' \umy T'$.
\end{lemma}
\begin{proof}
    It suffices to show that
    \[
        \srel \eqdef {\umy} \cup \set{ (S', T') \mid S \umy T \wedge S \lind{\inp\Tag} S' \wedge T \lmust{\inp\Tag} T'}
    \]
    is an ugly asynchronous subtyping.
    %
    Suppose $(S',T') \in \srel$. Then there exist $S$ and $T$ such that $S \umy
    T$ and $S \lind{\inp\Tag} S'$ and $T \lmust{\inp\Tag} T'$.
    %
    We prove the clauses of \Cref{def:umy} in order:
    \begin{enumerate}
    \item Suppose $S \lmust{\pol\unit}$. Then $S \lmust{\inp\Tag} S'
        \lmust{\pol\unit}$. From \umyref{inp} we deduce $S' \umy T'$, hence $T
        \lmust{\pol\unit}$ as required by \umyref{pol}.
    \item Suppose $S' \lmust{\inp\TagC}$. Then $S \lmust{\inp\Tag} S'
        \lmust{\inp\TagC}$. From \umyref{inp} we deduce $S' \umy T'$, hence $T'
        \lmust{\inp\TagB}$ and $T' \lmust{\inp\TagD} T''$ implies $S'
        \lmust{\inp\TagD} S''$ and $S'' \umy T''$ as required by \umyref{inp}.    
    \item Suppose $S' \lmust{\out\TagC} S''$. We distinguish two sub-cases.
        \begin{itemize}
        \item ($S \lmust{\inp\Tag} S'$) From \umyref{inp} we deduce $S' \umy
            T'$, hence $T' \lmust{\out\TagC} T''$ and $S'' \umy T''$ as required
            by \umyref{out}.
        \item ($S \lmust{\out\TagC} S'''$) From \umyref{out} we deduce $T
        \lind{\out\TagC} T'''$ and $S''' \umy T'''$. From \Cref{prop:diamond} we
        deduce $S''' \lind{\inp\Tag} S''$ and $T''' \lmust{\inp\Tag} T''$. We
        conclude $(S'',T'') \in \srel$ by definition of $\srel$.
        %
        \qedhere
        \end{itemize}
    \end{enumerate}
\end{proof}

\begin{theorem}
    ${\umy} \subseteq {\emy}$
\end{theorem}
\begin{proof}
    We show that $\umy$ is an elegant asynchronous subtyping assuming $S \umy T$
    and proving the clauses of \cref{def:emy} in order.
    \begin{enumerate}
    \item If $\positive(S)$ or $\negative(T)$, then \emyref{pol} is satisfied
        and there is nothing to prove. So suppose by contradiction that we have
        $\negative(S)$ and $\positive(T)$.
        %
        Suppose $S \lmust{\inp\unit}$. From \umyref{pol} we deduce $T
        \lmust{\inp\unit}$, which contradicts $\positive(T)$.
        %
        Suppose $S \lmust{\inp\TagB}$. From \umyref{out} we deduce $T
        \lmust{\inp\TagC}$, which contradicts $\positive(T)$.
        %
        We conclude that the hypothesis $\negative(S)$ and $\positive(T)$ is
        impossible.
    \item Suppose $T \lmust{\inp\MessageType} T'$. From
        \Cref{lem:umy-emy-late-input} we deduce $S \lind{\inp\MessageType} S'$
        for some $S'$.
        %
        From \Cref{lem:umy-emy-difficult-case} we deduce $S' \umy T'$, hence
        \emyref{inp} is satisfied.
    \item Suppose $S \lmust{\out\MessageType} S'$. We distinguish two sub-cases:
        \begin{itemize}
        \item ($\MessageType = \unit$) Then $S' = \One$. From \umyref{pol} we
            deduce $T \lmust{\out\unit} \One$. Hence \emyref{out} is satisfied.
        \item ($\MessageType = \Tag$) From \umyref{out} we deduce $T
            \lind{\out\Tag} T'$ and $S' \umy T'$, hence \emyref{out} is
            satisfied.
            %
            \qedhere
        \end{itemize}
    \end{enumerate}
\end{proof}
